Institutions, Education, and Religious Change: Evidence from Colombia

How do religious identities change? We study the effects of civic education reforms on religious identification using Colombia's 1991 Constitution, which dismantled the country's confessional regime and mandated constitutional instruction in high schools. Exploiting cohort-based variation in exposure to the reform and nationally representative survey data, we implement a difference-in-differences design. We find that exposure to the constitutional curriculum reduced Catholic self-identification by about three percentage points. This decline reflects a reallocation of religious identities rather than a generalized decline in religiosity. In regions where Catholic institutional presence was historically weaker, Catholic losses translate into switching toward non-Catholic Christian denominations and higher religious attendance. In contrast, in regions where Catholic dominance was stronger, the decline is associated with increased secular identification and lower attendance. These patterns hold across ethnic and non-ethnic groups and are shaped primarily by regional religious supply rather than ethnicity per se. Overall, the results show that civic education can reconfigure religious identities by reshaping the relative legitimacy of competing affiliations.

==> TABLE_atheist_paralleltrends_b10w2w3w4.tex <==
(Age $\leq$ 16 in 1984) $\times$ (Highschool)&       0.000         &       0.001         &      -0.000         \\
                    &     (0.001)         &     (0.001)         &     (0.001)         \\
                    &[-0.003 0.004]        &[-0.002 0.005]      &[-0.002 0.003]         \\
R-sq                &       0.005         &       0.004         &       0.004         \\
Observations        &       13084         &       18472         &       23535         \\


==> TABLE_atheist_paralleltrends_b2w2w3w4.tex <==
(Age $\leq$ 16 in 1992) $\times$ (Highschool)&      -0.000         &      -0.000         &       0.000         \\
                    &     (0.001)         &     (0.001)         &     (0.001)         \\
                    &[-0.003 0.010]          &[-0.001 0.007]        &[-0.001 0.006]         \\
R-sq                &       0.010         &       0.008         &       0.006         \\
Observations        &       13072         &       18577         &       24402         \\


==> TABLE_atheist_paralleltrends_b4w2w3w4.tex <==
(Age $\leq$ 16 in 1990) $\times$ (Highschool)&       0.001         &       0.002         &       0.002         \\
                    &     (0.001)         &     (0.002)         &     (0.001)         \\
                    &[-0.001 0.004]           &[-0.001 0.006]            &[-0.000 0.004]         \\
R-sq                &       0.007         &       0.006         &       0.007         \\
Observations        &       12920         &       18196         &       23520         \\


==> TABLE_atheist_paralleltrends_b6w2w3w4.tex <==
(Age $\leq$ 16 in 1988) $\times$ (Highschool)&       0.002         &       0.001         &       0.000         \\
                    &     (0.001)         &     (0.001)         &     (0.001)         \\
                    &[-0.004 0.004]     &[-0.006 0.003]              &[-0.005 0.002]         \\
R-sq                &       0.006         &       0.006         &       0.006         \\
Observations        &       12921         &       18350         &       23516         \\


==> TABLE_atheist_paralleltrends_b8w2w3w4.tex <==
(Age $\leq$ 16 in 1986) $\times$ (Highschool)&      -0.002         &      -0.002         &      -0.001         \\
                    &     (0.001)         &     (0.001)         &     (0.001)         \\
                    &[-0.003 0.002]               &[-0.003 0.002]      &[-0.002 0.003]         \\
R-sq                &       0.004         &       0.004         &       0.005         \\
Observations        &       13135         &       18245         &       23279         \\


==> TABLE_catholich_paralleltrends_b2w2w3_boot.tex <==
(Age $\leq$ 16 in 1992) $\times$ (Highschool)&      -0.021         &      -0.007         &      -0.038         &      -0.016         &       0.004         &      -0.038         &      -0.017         &      -0.012         &      -0.021         \\
                    &     (0.017)         &     (0.020)         &     (0.026)         &     (0.009)         &     (0.011)         &     (0.017)*        &     (0.008)         &     (0.010)         &     (0.009)*         \\
                    &[-0.051 0.041]            &[-0.064 0.043]            &[-0.109 0.034]           &[-0.033 0.015]        &[-0.042 0.021]         &[-0.068 0.005]          &[-0.032 0.011]    &[-0.032 0.021]      &[-0.037 0.026]         \\
R-sq                &       0.020         &       0.021         &       0.028         &       0.019         &       0.021         &       0.025         &       0.019         &       0.022         &       0.021         \\
Observations        &       13072         &        7115         &        5957         &       18577         &       10153         &        8424         &       24402         &       13220         &       11182         \\


==> TABLE_catholich_paralleltrends_b4w2w3_boot.tex <==
(Age $\leq$ 16 in 1990) $\times$ (Highschool)&       0.021         &       0.014         &       0.032         &       0.022         &       0.017         &       0.030         &       0.019         &       0.015         &       0.027         \\
                    &     (0.012)         &     (0.024)         &     (0.040)         &     (0.014)         &     (0.024)         &     (0.027)         &     (0.011)         &     (0.024)         &     (0.028)         \\
                    &[-0.007 0.093]     &[-0.062 0.182]     &[-0.028 0.164]   &[-0.013 0.115]        &[-0.036 0.188]     &[-0.008 0.113]       &[-0.004 0.102] &[-0.042 0.175]  &[-0.018 0.112]         \\
R-sq                &       0.020         &       0.022         &       0.026         &       0.019         &       0.019         &       0.026         &       0.018         &       0.020         &       0.022         \\
Observations        &       12920         &        7041         &        5879         &       18196         &        9876         &        8320         &       23520         &       12815         &       10705         \\


==> TABLE_catholich_paralleltrends_b6w2w3_boot.tex <==
(Age $\leq$ 16 in 1988) $\times$ (Highschool)&       0.003         &       0.006         &      -0.004         &       0.013         &       0.007         &       0.019         &       0.008         &      -0.000         &       0.020         \\
                    &     (0.014)         &     (0.019)         &     (0.012)         &     (0.011)         &     (0.015)         &     (0.014)         &     (0.011)         &     (0.016)         &     (0.011)         \\
                    &[-0.038 0.099]       &[-0.059 0.099]          &[-0.031 0.100]        &[-0.019 0.088]         &[-0.032 0.107]        &[-0.035 0.061]    &[-0.016 0.091]    &[-0.032 0.118]    &[-0.021 0.065]         \\
R-sq                &       0.015         &       0.020         &       0.019         &       0.017         &       0.020         &       0.021         &       0.018         &       0.021         &       0.022         \\
Observations        &       12921         &        7046         &        5875         &       18350         &        9964         &        8386         &       23516         &       12843         &       10673         \\


==> TABLE_catholich_paralleltrends_b8w2w3_boot.tex <==
(Age $\leq$ 16 in 1986) $\times$ (Highschool)&      -0.004         &      -0.012         &       0.007         &      -0.007         &      -0.013         &       0.002         &      -0.011         &      -0.012         &      -0.008         \\
                    &     (0.011)         &     (0.019)         &     (0.022)         &     (0.014)         &     (0.016)         &     (0.027)         &     (0.012)         &     (0.016)         &     (0.022)         \\
                    &[-0.027 0.037]       &[-0.045 0.041]         &[-0.063 0.040]       &[-0.063 0.037]          &[-0.067 0.039]     &[-0.076 0.043]      &[-0.045 0.021]    &[-0.035 0.039]   &[-0.068 0.027]         \\
R-sq                &       0.019         &       0.027         &       0.022         &       0.017         &       0.022         &       0.019         &       0.016         &       0.019         &       0.019         \\
Observations        &       13135         &        7157         &        5978         &       18245         &        9983         &        8262         &       23279         &       12743         &       10536         \\


==> TABLE_noreligion_paralleltrends_b10w2w3w4.tex <==
(Age $\leq$ 16 in 1984) $\times$ (Highschool)&       0.009         &       0.007         &       0.004         \\
                    &     (0.005)         &     (0.005)         &     (0.003)         \\
                    &[0.001 0.041]***         &[-0.004 0.043]           &[-0.003 0.022]         \\
R-sq                &       0.016         &       0.016         &       0.016         \\
Observations        &       13084         &       18472         &       23535         \\


==> TABLE_noreligion_paralleltrends_b2w2w3w4.tex <==
(Age $\leq$ 16 in 1992) $\times$ (Highschool)&      -0.000         &      -0.000         &       0.000         \\
                    &     (0.010)         &     (0.007)         &     (0.007)         \\
                    &[-0.021 0.019]         &[-0.015 0.016]        &[-0.016 0.015]         \\
R-sq                &       0.016         &       0.015         &       0.013         \\
Observations        &       13072         &       18577         &       24402         \\


==> TABLE_noreligion_paralleltrends_b4w2w3w4.tex <==
(Age $\leq$ 16 in 1990) $\times$ (Highschool)&      -0.007         &      -0.011         &      -0.014         \\
                    &     (0.007)         &     (0.004)\sym{*}  &     (0.003)\sym{*}  \\
                    &[-0.031 0.017]          &[-0.023 -0.005]***           &[-0.021 -0.007]***         \\
R-sq                &       0.015         &       0.015         &       0.015         \\
Observations        &       12920         &       18196         &       23520         \\


==> TABLE_noreligion_paralleltrends_b6w2w3w4.tex <==
(Age $\leq$ 16 in 1988) $\times$ (Highschool)&      -0.006         &      -0.013         &      -0.014         \\
                    &     (0.008)         &     (0.006)         &     (0.006)         \\
                    &[-0.055 0.017]          &[-0.042 0.010]*        &[-0.047 0.006]*         \\
R-sq                &       0.015         &       0.014         &       0.015         \\
Observations        &       12921         &       18350         &       23516         \\


==> TABLE_noreligion_paralleltrends_b8w2w3w4.tex <==
(Age $\leq$ 16 in 1986) $\times$ (Highschool)&      -0.009         &      -0.008         &      -0.004         \\
                    &     (0.006)         &     (0.007)         &     (0.003)         \\
                    &[-0.026 -0.001]**        &[-0.035 0.001]         &[-0.012 0.003]         \\
R-sq                &       0.016         &       0.014         &       0.014         \\
Observations        &       13135         &       18245         &       23279         \\


==> TABLE_othchrtncath_paralleltrends_b10w2w3w4.tex <==
(Age $\leq$ 16 in 1984) $\times$ (Highschool)&       0.001         &      -0.000         &       0.002         \\
                    &     (0.003)         &     (0.003)         &     (0.002)         \\
                    &[-0.011 0.008]             &[-0.010 0.009]         &[-0.009 0.009]         \\
R-sq                &       0.006         &       0.007         &       0.005         \\
Observations        &       13084         &       18472         &       23535         \\


==> TABLE_othchrtncath_paralleltrends_b2w2w3w4.tex <==
(Age $\leq$ 16 in 1992) $\times$ (Highschool)&       0.003         &       0.000         &      -0.001         \\
                    &     (0.005)         &     (0.004)         &     (0.003)         \\
                    &[-0.009 0.042]           &[-0.012 0.030]          &[-0.013 0.017]         \\
R-sq                &       0.004         &       0.003         &       0.003         \\
Observations        &       13072         &       18577         &       24402         \\


==> TABLE_othchrtncath_paralleltrends_b4w2w3w4.tex <==
(Age $\leq$ 16 in 1990) $\times$ (Highschool)&      -0.003         &      -0.003         &      -0.001         \\
                    &     (0.003)         &     (0.004)         &     (0.003)         \\
                    &[-0.022 0.001]          &[-0.017 0.004]       &[-0.014 0.005]         \\
R-sq                &       0.004         &       0.004         &       0.003         \\
Observations        &       12920         &       18196         &       23520         \\


==> TABLE_othchrtncath_paralleltrends_b6w2w3w4.tex <==
(Age $\leq$ 16 in 1988) $\times$ (Highschool)&       0.003         &       0.001         &       0.003         \\
                    &     (0.002)         &     (0.003)         &     (0.002)         \\
                    &[-0.017 0.007]          &[-0.019 0.009]          &[-0.008 0.007]         \\
R-sq                &       0.004         &       0.004         &       0.004         \\
Observations        &       12921         &       18350         &       23516         \\


==> TABLE_othchrtncath_paralleltrends_b8w2w3w4.tex <==
(Age $\leq$ 16 in 1986) $\times$ (Highschool)&       0.005         &       0.004         &       0.004         \\
                    &     (0.003)         &     (0.004)         &     (0.003)         \\
                    &[-0.002 0.027]        &[-0.006 0.016]       &[-0.005 0.012]         \\
R-sq                &       0.005         &       0.005         &       0.004         \\
Observations        &       13135         &       18245         &       23279         \\


==> TABLE_protesevan_paralleltrends_b10w2w3w4.tex <==
(Age $\leq$ 16 in 1984) $\times$ (Highschool)&       0.004         &      -0.001         &      -0.000         \\
                    &     (0.009)         &     (0.007)         &     (0.010)         \\
                    &[-0.015 0.036]        &[-0.018 0.017]     &[-0.018 0.055]         \\
R-sq                &       0.013         &       0.013         &       0.014         \\
Observations        &       13084         &       18472         &       23535         \\


==> TABLE_protesevan_paralleltrends_b2w2w3w4.tex <==
(Age $\leq$ 16 in 1992) $\times$ (Highschool)&       0.015         &       0.016         &       0.021         \\
                    &     (0.011)         &     (0.006)         &     (0.009)         \\
                    &[-0.010 0.058]      &[0.006 0.037]***       &[-0.020 0.048]*         \\
R-sq                &       0.016         &       0.014         &       0.015         \\
Observations        &       13072         &       18577         &       24402         \\


==> TABLE_protesevan_paralleltrends_b4w2w3w4.tex <==
(Age $\leq$ 16 in 1990) $\times$ (Highschool)&      -0.007         &      -0.005         &      -0.003         \\
                    &     (0.005)         &     (0.012)         &     (0.009)         \\
                    &[-0.050 0.009]         &[-0.054 0.038]            &[-0.037 0.029]         \\
R-sq                &       0.014         &       0.014         &       0.013         \\
Observations        &       12920         &       18196         &       23520         \\


==> TABLE_protesevan_paralleltrends_b6w2w3w4.tex <==
(Age $\leq$ 16 in 1988) $\times$ (Highschool)&      -0.001         &      -0.001         &       0.004         \\
                    &     (0.007)         &     (0.005)         &     (0.007)         \\
                    &[-0.027 0.013]        &[-0.017 0.016]        &[-0.011 0.024]         \\
R-sq                &       0.011         &       0.012         &       0.012         \\
Observations        &       12921         &       18350         &       23516         \\


==> TABLE_protesevan_paralleltrends_b8w2w3w4.tex <==
(Age $\leq$ 16 in 1986) $\times$ (Highschool)&       0.009         &       0.009         &       0.008         \\
                    &     (0.006)         &     (0.008)         &     (0.010)         \\
                    &[-0.005 0.023]     &[-0.004 0.041]       &[-0.010 0.037]         \\
R-sq                &       0.012         &       0.012         &       0.012         \\
Observations        &       13135         &       18245         &       23279         \\


==> table_atheist_all.tex <==

(Age $\leq$ 16 in 1994) $\times$ (Highschool)&       0.000         &       0.000         &       0.001         \\
                    &     (0.002)         &     (0.002)         &     (0.002)         \\
                    &[-0.004 0.004]           &[-0.004 0.005]        &[-0.003 0.004]         \\
R-sq                &       0.000         &       0.003         &       0.007         \\
Observations        &       19875         &       19875         &       19875         \\


==> table_christnoncath_all.tex <==
(Age $\leq$ 16 in 1994) $\times$ (Highschool)&       0.025         &       0.026         &       0.030         \\
                    &     (0.007)\sym{**}  &     (0.008)\sym{**}  &     (0.010)\sym{**}  \\
                    &[-0.003 0.043]*       &[-0.004 0.046]**             &[0.011 0.050]***         \\
R-sq                &       0.001         &       0.012         &       0.022         \\
Observations        &       20356         &       20356         &       20356         \\


==> table_noreligion_all.tex <==
(Age $\leq$ 16 in 1994) $\times$ (Highschool)&       0.014         &       0.014         &       0.015         \\
                    &     (0.009)         &     (0.008)         &     (0.008)         \\
                    &[-0.004 0.044]*         &[-0.002 0.044]*            &[-0.001 0.040]*         \\
R-sq                &       0.001         &       0.007         &       0.015         \\
Observations        &       19875         &       19875         &       19875         \\


==> table_otherchristiannocatholic_all.tex <==
(Age $\leq$ 16 in 1994) $\times$ (Highschool)&       0.002         &       0.003         &       0.002         \\
                    &     (0.003)         &     (0.003)         &     (0.003)         \\
                    &[-0.003 0.009]                  &[-0.003 0.010]          &[-0.003 0.009]         \\
R-sq                &       0.000         &       0.001         &       0.003         \\
Observations        &       19875         &       19875         &       19875         \\


==> table_protentantevangelical_all.tex <==
(Age $\leq$ 16 in 1994) $\times$ (Highschool)&       0.012         &       0.012         &       0.016         \\
                    &     (0.012)         &     (0.011)         &     (0.012)         \\
                    &[-0.032 0.042]                 &[-0.031 0.040]         &         [-0.020 0.046]         \\
R-sq                &       0.000         &       0.009         &       0.017         \\
Observations        &       19875         &       19875         &       19875         \\


==> table_region25_noreg1.tex <==
(Age $\leq$ 16 in 1994) $\times$ (High school) & -0.032 & 0.030 & 0.002 & 0.000 & 0.030 \\
  & (0.012) & (0.019) & (0.006) & (0.001) & (0.011) \\
  & [-0.046, -0.021]*** & [0.012, 0.052]*** & [-0.005, 0.008] & [-0.001, 0.001] & [0.018, 0.041]*** \\
R-sq  & 0.026 & 0.019 & 0.003 & 0.015 & 0.062 \\
Observations  & 9,333 & 9,333 & 9,333 & 9,333 & 3,486 \\


==> table_religiosity.tex <==
(Age $\leq$ 16 in 1994) $\times$ (Highschool)&       0.041   &       0.036   &       0.044   \\
                    &     (0.037)   &     (0.057)   &     (0.046)   \\
                    &[-0.038 0.126]       &[-0.147 0.348]        &[-0.411 0.177]   \\
R-sq                &       0.056   &       0.054   &       0.043   \\
Observations        &       12071   &        6418   &        5653   \\

